A Study of Undefined Behavior Across Foreign Function Boundaries in Rust Libraries

Developers rely on the static safety guarantees of the Rust programming language to write secure and performant applications. However, Rust is frequently used to interoperate with other languages which allow design patterns that conflict with Rust's evolving aliasing models. Miri is currently the only dynamic analysis tool that can validate applications against these models, but it does not support finding bugs in foreign functions, indicating that there may be a critical correctness gap across the Rust ecosystem. We conducted a large-scale evaluation of Rust libraries that call foreign functions to determine whether Miri's dynamic analyses remain useful in this context. We used Miri and an LLVM interpreter to jointly execute applications that call foreign functions, where we found 46 instances of undefined or undesired behavior in 37 libraries. Three bugs were found in libraries that had more than 10,000 daily downloads on average during our observation period, and one was found in a library maintained by the Rust Project. Many of these bugs were violations of Rust's aliasing models, but the latest Tree Borrows model was significantly more permissive than the earlier Stacked Borrows model. The Rust community must invest in new, production-ready tooling for multi-language applications to ensure that developers can detect these errors.

==> figures/asptr.tex <==
\begin{rustfigure}
pub fn as_ffi(&self) -> *mut T {
    self.data.as_ref() as *const T as *mut T |\label{asptr:cast}|
}
\end{rustfigure}




==> figures/const_correctness.tex <==

\begin{rustfigure}
pub struct Settings {
  data: Box<Data>,
}
pub fn as_ffi(&self) -> *mut T {
  self.data.as_ref() as *const T <<^as *mut T^>>
}
\end{rustfigure}

\begin{rustfigure}
pub struct Settings {
  data: <<@NonNull<Data>@>>,
}
pub fn as_ffi(&self) -> *mut T {
  <<@self.data.as_ptr()@>>
}
\end{rustfigure}


==> figures/maybeuninit_decnumber.tex <==
\begin{rustfigure}
let mut d = MaybeUninit::<[u32;2]>::uninit();
let d = unsafe {
  ffi::init(d.as_mut_ptr() as *mut u32);
  d.assume_init()
};
\end{rustfigure}
\begin{ccfigure}
void init(uint32_t * x) {
  *data = 0
}
\end{ccfigure}

==> figures/maybeuninit_xxhrs.tex <==
\begin{subcaptionblock}[T]{.5\textwidth}
\caption{The function \code{init} is implemented in C (top) and compiles to LLVM IR (bottom). The LLVM representation leaves the parameter \code{s} partially initialized, since it is not fully copied out by \code{memcpy}.}
\begin{rustfigure}
void init(state_t* s) {
  memset(s, 0, sizeof(*s));|\label{padding:original}|
}
\end{rustfigure}
\begin{rustfigure}
define void @init(ptr %0) {
  %1 = alloca %struct.state_t
  call void @memset(ptr %1, i8 0, i64 88) |\label{padding:llvm:set}|
  call void @memcpy(ptr %0, ptr %1, <<^i64 80^>>) |\label{padding:llvm:get}|
}
\end{rustfigure}
\end{subcaptionblock} \hfill\begin{subcaptionblock}[T]{.45\textwidth}
\caption{The bug was fixed by manually initializing the padding field in Rust.}
\begin{rustfigure}
let mut state = MaybeUninit::uninit();
unsafe {
  ffi::init(state.as_mut_ptr()); 
  <<@(*state).padding = 0;@>>
  return state.assume_init();
}
\end{rustfigure}
\end{subcaptionblock}

==> figures/oob.tex <==
\begin{rustfigure}
<<^- let x = CString::new(Vec::with_capacity(4))^>>
  <<^- .map_err(...)?^>>
  <<^- .into_raw();^>>
<<@+ let x = b"    ".to_vec();@>>
unsafe {
<<@+ let x = CString::from_vec_unchecked(text)@>>
  <<@+ .into_raw();@>>
  ffi(x);
  CString::from_raw(x)
};
\end{rustfigure}

==> figures/phantomdata.tex <==
\begin{rustfigure}
<<^- struct CType(PhantomData<UnsafeCell<*mut ()>>);^>>
<<@+ struct CType(UnsafeCell<*mut ()>>);@>>
  fn as_ptr(&self) -> *mut Self::CType {
    <<^- self as *const _ as *mut _^>>
    <<@+ self.get()@>>
  }
\end{rustfigure}

==> highlighter.tex <==
% Credit: https://tex.stackexchange.com/a/49309
\makeatletter
\@ifpackageloaded{tikz}{}{\usepackage{tikz}}
\@ifpackageloaded{listings}{}{\usepackage{listings}}
\newenvironment{btHighlight}[1][]
{\begingroup\tikzset{bt@Highlight@par/.style={#1}}\begin{lrbox}{\@tempboxa}}
{\end{lrbox}\bt@HL@box[bt@Highlight@par]{\@tempboxa}\endgroup}

\newcommand\btHL[1][]{%
  \begin{btHighlight}[#1]\bgroup\aftergroup\bt@HL@endenv%
}
\def\bt@HL@endenv{%
  \end{btHighlight}%   
  \egroup
}
\newcommand{\bt@HL@box}[2][]{%
  \tikz[#1]{%
    \pgfpathrectangle{\pgfpoint{1pt}{0pt}}{\pgfpoint{\wd #2}{\ht #2}}%
    \pgfusepath{use as bounding box}%
    \node[anchor=base west, fill=orange!30,outer sep=0pt,inner xsep=1pt, inner ysep=0pt, rounded corners=3pt, minimum height=\ht\strutbox+1pt,#1]{\raisebox{1pt}{\strut}\strut\usebox{#2}};
  }%
}
\makeatother
